Contracts for Abstract Processes in Service Composition

Contracts are a well-established approach for describing and analyzing behavioral aspects of web service compositions. The theory of contracts comes equipped with a notion of compatibility between clients and servers that ensures that every possible interaction between compatible clients and servers will complete successfully. It is generally agreed that real applications often require the ability of exposing just partial descriptions of their behaviors, which are usually known as abstract processes. We propose a formal characterization of abstraction as an extension of the usual symbolic bisimulation and we recover the notion of abstraction in the context of contracts.

==> eptcsdata.tex <==
\providecommand{\firstpage}{9}
\providecommand{\publicationstatus}{Beno\^it Caillaud and Axel Legay (Eds.):\\
Foundations of Interface Technologies (FIT'10)\\
EPTCS 46, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.46.2}{10.4204/EPTCS.46.2}}
\pdfoutput=1

